Refining and Delegating Strategic Ability in ATL

We propose extending Alternating-time Temporal Logic (ATL) by an operator <i refines-to G> F to express that agent i can distribute its powers to a set of sub-agents G in a way which satisfies ATL condition f on the strategic ability of the coalitions they may form, possibly together with others agents. We prove the decidability of model-checking of formulas whose subformulas with this operator as the main connective have the form <i_1 refines-to G_1>...<i_m refines-to G_m> f, with no further occurrences of this operator in f.

==> eptcsdata.tex <==
\providecommand{\firstpage}{57}
\providecommand{\publicationstatus}{F. Mogavero, A. Murano, and M.Y. Vardi (Eds.): \\
2nd Workshop on Strategic Reasoning 2014 (SR'14)\\
EPTCS 146, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.146.8}{10.4204/EPTCS.146.8}}

